IoTGaze: IoT Security Enforcement via Wireless Context Analysis

Internet of Things (IoT) has become the most promising technology for service automation, monitoring, and interconnection, etc. However, the security and privacy issues caused by IoT arouse concerns. Recent research focuses on addressing security issues by looking inside platform and apps. In this work, we creatively change the angle to consider security problems from a wireless context perspective. We propose a novel framework called IoTGaze, which can discover potential anomalies and vulnerabilities in the IoT system via wireless traffic analysis. By sniffing the encrypted wireless traffic, IoTGaze can automatically identify the sequential interaction of events between apps and devices. We discover the temporal event dependencies and generate the Wireless Context for the IoT system. Meanwhile, we extract the IoT Context, which reflects user's expectation, from IoT apps' descriptions and user interfaces. If the wireless context does not match the expected IoT context, IoTGaze reports an anomaly. Furthermore, IoTGaze can discover the vulnerabilities caused by the inter-app interaction via hidden channels, such as temperature and illuminance. We provide a proof-of-concept implementation and evaluation of our framework on the Samsung SmartThings platform. The evaluation shows that IoTGaze can effectively discover anomalies and vulnerabilities, thereby greatly enhancing the security of IoT systems.

==> nlp_summary.tex <==
\section{Natural language processing}

1. User expectations and application functionality \\
2. Does the application description provide any indication for the application's use of a permission? \\
3. application name, users reviews, and potentially even screen-shots \\
4. creating and fine-tuning permission semantic models \\
5. Confounding effects \\
6. Semantic inference, use API documents to identify actions and resources \\
7. Key NLP techniques: parts of speech tagging, phrase and clause parsing, typed dependencies and named entity recognition

\section{smartAuth}

There exists a crucial gap between a user believe an IoT app will do, and what the app actually does?\\
SmartAuth learns about each IoT app's actual functionality by automatically harvesting and analyzing information from sources, such as the app's source code, code annotations, and capability requests.\\

https://github.com/SmartThingsCommunity/SmartThingsPublic

NLP technologies used:
Word2Vec is a state-of-the-art tool used to produce word embedding that maps words to vectors of real numbers.\\
Word2Vec determines the relation between two words by caculating the distance between the words in the embedding space.\\
Part-of-speech tagging is used to identify a word's part of speech(e.g., noun or verb) based on definition and context.Standford POS Tagger\\
Typed dependencies analysis understand the grammatical structures of sentences, grouping words together to recognize phrases and pair subjects or objects with verbs.

\subsection{analyzing app descriptions}
1. use the Stanford POS Tagger to identify parts of speech
2. use stanford parser to analyze sentence structure, including typed dependencies
3. analyze the noun and verb phrases to pinpoint the relevant entities, as these phrases usually describe core app functionality.
4. The most straightforward case is when the description explicitly includes the name of the entity, if so, just match words directly
5. most time, we cannot find the words directly matched. However

\section{HoMoNit}
Extracting DFA without source code is more challenging since the descriptions of the SmartApps are usually very simple(e.g., only one sentence). So we leverage the text embedded in the user interface of the SmartThings mobile app to extract the logic of the SmartApps to build its DFA.
(1). Text extraction.\\
Extract the text value in the XML code from the Android App UI,
such as $<text="when\ water\ is\ sensed.">$. still do not know the related the sensors that the app uses. go to the next step.

(2). Symbol inference.\\
infer associated commands or attributes of capabilities form the extracted text. The UI interface prompts the user to select the devices that have the corresponding capabilities requested by the SmartApp. There are 72 capabilities defined in the SmartThings Developer documents. If the size of the candidate set from the drop-down list is only 1, that means we do not need to infer the capabilities via the NLP techniques.

If the candidate size is more than one, NLP analysis is needed to further reduce the candidate set. HoMoNIT use NLTK to extract the noun phrases and verb phrases in a sentence. 

Capabilities are often related to the noun phrases in the text. The HoMoNIT compares the noun phrases with capability candidate set and uses text simlarity(estimated by Word2Vec) to determine the requested capability. We combine Word2Vec with a model trained with the API documentation of SmartThings.

After learning the requested capabilities, the next step is to find out the exact attributes or commands of the capability. obtain the possible attributes or commands of each capability from the official documentation, and analyze the verb phrases to conduct the inference. Use Word2Vec to analyze the context of the verb phrases. For example, for switch capability, there are two commands: on() and off(), and the verb phrase turn on is more likely to be linked to the on() command.

(3). DFA building
chainning the commands or attributes according to the text, which describe the logical relationship.

\section{Identification of Similar IoT apps via activity footprints}


\section{IoTMON}
The physical interaction capabilities enable devices to interact with each other through shared physical environments.

IoTMON captures all potential physical interactions across applications and enable safe interaction controls on IoT platform. \\
Three steps: (1): application analysis. (2) interaction chain discovery. (3) risk analysis & mitigation.

Application analysis: Intra-app analysis General IoT application follows the "If-This-Then-That"(IFTTT) programming paradigm. "This" corresponds to the trigger capability and condition threshold. "That" represents the triggered action, such as changing a device's status.

Physical Channel Identification: 1. Use NLP techniques to extract channel entity keywords from application descriptions.(use the Stanford NLP tool) to parse the description.
2. Calculate similarities of extracted keywords by using Word2Vec with a widely used language model (Google News Vectors). 3. Based on the similarities of entity keywords, we cluster those entity keywords and identify physical channels based on entity keyword clusters.

\section{other relevant papers}
1. Checking App Behavior Against App Descriptions\\
2. AutoCog: Measuring the Description-to-permission Fidelity in Android Applications.\\
3. FlowCog: Context-aware Semantics Extraction and Analysis of Information Flow Leaks in Android Apps\\
4. IOTGUARD: Dynamic Enforcement of Security and Safety Policy in Commodity IoT.\\

5. relevant NLP technique may be leveraged

1). Semantic Textual Similarity (STS) measures the degree of equivalence in the underlying semantics of paired snippets of text. (https://github.com/rgtjf/Semantic-Texual-Similarity-Toolkits).

2). Relationship Extraction. 
Relationship extraction is the task of extracting semantic relationships from a text. Extracted relationships usually occur between two or more entities of a certain type (e.g. Person, Organisation, Location) and fall into a number of semantic categories (e.g. married to, employed by, lives in).

3). Part-of-speech tagging. 
Part-of-speech tagging (POS tagging) is the task of tagging a word in a text with its part of speech. A part of speech is a category of words with similar grammatical properties. Common English parts of speech are noun, verb, adjective, adverb, pronoun, preposition, conjunction, etc.

4). Semantic parsing. 
Semantic parsing is the task of translating natural language into a formal meaning representation on which a machine can act. Representations may be an executable language such as SQL or more abstract representations such as Abstract Meaning Representation (AMR).

==> table_back_up.tex <==
%-------following is the code for the first table--------
\begin{table*}[t]
\centering
\begin{tabular}[c]{|M{0.4cm}|M{12.6cm}|M{3.4cm}|}
\hline
\textbf{No.} & \textbf{Event chain}             & \textbf{symbol representation} \\ \hline
1   
& \framebox[1.1\width]{motion sensor}$\xrightarrow{\text{active}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light} 
&  $\circled{\small 1}\xrightarrow{}\circled{\small 2}$  
\\   
\cline{2-3}
& \textcolor{red}{\framebox[1.1\width]{motion sensor}}\textcolor{red}{$\xrightarrow{\text{\st{active}}}$} \framebox[1.1\width]{hub} $\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light} 
&  \textcolor{red}{\sout{\circled{\small 1}}} $\xrightarrow{} \circled{\small 2}$  
\\ \hline
% 2   & \framebox[1.1\width]{water sensor}$\xrightarrow{\text{wet}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{valve.close()}}$ \framebox[1.1\width]{valve}                     &   $\circled{\small 3}\xrightarrow{}\circled{\small 4}$                    &     2      \\ \hline
2   
& \framebox[1.1\width]{temperature sensor}$\xrightarrow{\text{temperature}>\text{threshold}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{window.open()}}$ \framebox[1.1\width]{window}               
&  $\circled{\small 3}\xrightarrow{}\circled{\small 4}$                  
\\   
\cline{2-3}
& \framebox[1.1\width]{temperature sensor}\textcolor{red}{$\xrightarrow{\text{\st{temperature > threshold}}}$} \framebox[1.1\width]{hub} $\xrightarrow{\text{window.open()}}$ \framebox[1.1\width]{window} 
&  \textcolor{red}{\sout{\circled{\small 3}}}$\xrightarrow{}\circled{\small 4}$ 
\\ \hline
3   
& \framebox[1.1\width]{presence sensor}$\xrightarrow{\text{not present}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{camera.on()}}$ \framebox[1.1\width]{camera}                        
& $\circled{\small 5}\xrightarrow{}\circled{\small 6}$                 
\\   
\cline{2-3}
& \framebox[1.1\width]{presence sensor}$\xrightarrow{\text{not present}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{camera.on()}}$ \framebox[1.1\width]{camera} \textcolor{red}{$\xrightarrow{\text{camera.off()}}$ \framebox[1.1\width]{camera}}
& $\circled{\small 5}\xrightarrow{}\circled{\small 6}\enspace\textcolor{red}{\xrightarrow{}\circled{\small 7}}$ 
\\ \hline
4   
& \framebox[1.1\width]{door lock}$\xrightarrow{\text{unlocked}}$ \framebox[1.1\width]{hub},  \framebox[1.1\width]{contact sensor}$\xrightarrow{\text{open}}$ \framebox[1.1\width]{hub}, \framebox[1.1\width]{motion sensor}$\xrightarrow{\text{active}}$ \framebox[1.1\width]{hub}          
& $\circled{\small 8}\xrightarrow{}\circled{\small 9}\xrightarrow{}\circled{\small 1}$                
\\ 
\cline{2-3}
& \framebox[1.1\width]{door lock}$\xrightarrow{\text{unlocked}}$ \framebox[1.1\width]{hub},  \textcolor{red}{\framebox[1.1\width]{contact sensor}$\xrightarrow{\text{\st{open}}}$ \framebox[1.1\width]{hub}}, \framebox[1.1\width]{motion sensor}$\xrightarrow{\text{active}}$ \framebox[1.1\width]{hub} 
& \circled{\small 8}$\xrightarrow{}$\textcolor{red}{\sout{\circled{\small 9}}}$\xrightarrow{}\circled{\small 1}$   
\\ \hline
% 6   & \framebox[1.1\width]{smoke detector}$\xrightarrow{\text{detected}}$ \framebox[1.1\width]{hub}$\bm{\{}\xrightarrow{\text{unlock()}}$ \framebox[1.1\width]{door lock}, $\xrightarrow{\text{alarm.siren()}}$ \framebox[1.1\width]{alarm}\enspace $\bm{\}}$                        &               $\circled{\scriptsize 11}\xrightarrow{}\bm{\{}\circled{\scriptsize 12}, \enspace\circled{\scriptsize 13}\bm{\}}$        &     3     \\ \hline
5   
& $\bm{\{}$ \framebox[1.1\width]{contact sensor} $\xrightarrow{\text{open}}$, \framebox[1.1\width]{illuminance sensor} $\xrightarrow{\text{illuminance}<\text{threshold}}$ $\bm{\}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{hallway light}          
&   $\bm{\{}\circled{\small 9}, \enspace\circled{\scriptsize 10}\bm{\}}\xrightarrow{}\circled{\scriptsize 11}$
\\ 
\cline{2-3}
& $\bm{\{}$ \framebox[1.1\width]{contact sensor} $\xrightarrow{\text{open}}$, \framebox[1.1\width]{illuminance sensor} $\xrightarrow{\text{illuminance}<\text{threshold}}$ $\bm{\}}$ \framebox[1.1\width]{hub} \textcolor{red}{$\xrightarrow{\text{switch.off()}}$ \framebox[1.1\width]{hallway light}}  
&   $\bm{\{}\circled{\small 9}, \enspace\circled{\scriptsize 10}\bm{\}}\xrightarrow{}\textcolor{red}{\circled{\scriptsize 12}}$
\\ \hline
6   
& \framebox[1.1\width]{hub} $\xrightarrow{\text{switch.on()}}$\framebox[1.1\width]{hallway light}, \framebox[1.1\width]{hub} $\xrightarrow{\text{switch.off()}}$\framebox[1.1\width]{livingroom light}, \framebox[1.1\width]{hub} $\xrightarrow{\text{switch.off()}}$\framebox[1.1\width]{hallway light}      
&   $\circled{\scriptsize 11}\xrightarrow{}\circled{\scriptsize 13}\xrightarrow{}\circled{\scriptsize 12}$ 
\\ 
\cline{2-3}
& \framebox[1.1\width]{hub} $\xrightarrow{\text{on()}}$\framebox[1.1\width]{hallway light}, \framebox[1.1\width]{hub} $\xrightarrow{\text{off()}}$\framebox[1.1\width]{livingroom light}, \framebox[1.1\width]{hub} $\xrightarrow{\text{off()}}$\framebox[1.1\width]{hallway light}, \textcolor{red}{\framebox[1.1\width]{hub} $\xrightarrow{\text{unlock()}}$ \framebox[1.1\width]{door lock}}
&   $\circled{\scriptsize 11}\xrightarrow{}\circled{\scriptsize 13}\xrightarrow{}\circled{\scriptsize 12}\enspace\textcolor{red}{\xrightarrow{}\circled{\scriptsize 14}}$
\\ \hline
7   
& $\bm{\{}$ \framebox[1.1\width]{presence sensor} $\xrightarrow{\text{not present}}$, \framebox[1.1\width]{contact sensor} $\xrightarrow{\text{closed}}$, \framebox[1.1\width]{door lock} $\xrightarrow{\text{unlocked}}$  $\bm{\}}$  \framebox[1.1\width]{hub} $\xrightarrow{\text{lock.lock()}}$ \framebox[1.1\width]{door lock}               
& $\bm{\{}\circled{\small 5}, \enspace\circled{\scriptsize 15},\enspace \circled{\small 8}\bm{\}}\xrightarrow{} \circled{\scriptsize 16}$                 
\\ 
\cline{2-3}
& $\bm{\{}$ \framebox[1.1\width]{presence sensor} $\xrightarrow{\text{not present}}$, \framebox[1.1\width]{contact sensor} $\xrightarrow{\text{closed}}$, \framebox[1.1\width]{door lock} $\xrightarrow{\text{unlocked}}$  $\bm{\}}$  \framebox[1.1\width]{hub} \textcolor{red}{$\xrightarrow{\text{\st{lock.lock()}}}$ \framebox[1.1\width]{door lock}}               
& $\bm{\{}\circled{\small 5}, \enspace\circled{\scriptsize 15},\enspace \circled{\small 8}\bm{\}}\xrightarrow{}$ \textcolor{red}{\sout{\circled{\scriptsize 16}}} 
\\ \hline
8  
& $\bm{\{}$ \framebox[1.1\width]{presence sensor} $\xrightarrow{\text{present}}$, \framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}<\text{thresh}}$ $\bm{\}}$ \framebox[1.1\width]{hub} $\bm{\{}$ $\xrightarrow{\text{color.set(`blue')}}$ \framebox[1.1\width]{hue}, $\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{heater}   $\bm{\}}$           
&  $\bm{\{}\circled{\scriptsize 17}, \enspace\circled{\small 3}\bm{\}}\xrightarrow{} \bm{\{}\circled{\scriptsize 18}, \enspace \circled{\scriptsize 19}\bm{\}}$          
\\ 
\cline{2-3}
& $\bm{\{}$ \framebox[1.1\width]{presence sensor} $\xrightarrow{\text{present}}$, \framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}<\text{thresh}}$ $\bm{\}}$ \framebox[1.1\width]{hub} $\bm{\{}$ $\xrightarrow{\text{color.set(`blue')}}$ \framebox[1.1\width]{hue}, \textcolor{red}{$\xrightarrow{\text{\st{switch.on()}}}$ \framebox[1.1\width]{heater}}   $\bm{\}}$ 
&  $\bm{\{}\circled{\scriptsize 17}, \enspace\circled{\small 3}\bm{\}}\xrightarrow{} \bm{\{}\circled{\scriptsize 18},$ \textcolor{red}{\sout{\circled{\scriptsize 19}}} $\bm{\}}$
\\ \hline
\end{tabular}
\caption{Chain of multiple events}
\end{table*}

% \begin{table*}[t]
% \centering
% \begin{tabular}[c]{|M{0.3cm}|M{14.2cm}|M{0.8cm}|M{1.1cm}|}
% \hline
% \textbf{No.} & \textbf{Event chain}             & \textbf{\#apps} & \textbf{\#channels} \\ \hline
% 1   & \dashedbox{\framebox[1.1\width]{time}$\xrightarrow{}$\framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{toaster}} $\xrightarrow{}$ \cfbox{blue}{smoke} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{smoke detector} $\xrightarrow{\text{detected}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{alarm.siren()}}$ \framebox[1.1\width]{alarm}} &   2  & 1         \\ \hline
% 2   & \dashedbox{\framebox[1.1\width]{time}$\xrightarrow{}$\framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{heater}} $\xrightarrow{}$ \cfbox{blue}{temperature} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}>\text{thresh}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{window.open()}}$ \framebox[1.1\width]{window}} &   2  & 1         \\ \hline
% 3   & \dashedbox{\framebox[1.1\width]{presence sensor}$\xrightarrow{\text{not present}}$ \framebox[1.1\width]{hub}} $\xrightarrow{}$ \cfbox{blue}{location mode} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{hub} $\xrightarrow{\text{switch.off()}}$ \framebox[1.1\width]{light}} &   2  & 1         \\ \hline
% 4   & \dashedbox{\framebox[1.1\width]{humidity sensor} $\xrightarrow{\text{humidity}<\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{humidifier}} $\xrightarrow{}$ \cfbox{blue}{humidity} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{water sensor} $\xrightarrow{\text{wet}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}} &   2  & 1         \\ \hline
% 5   & \dashedbox{\framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}<\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{fan}} $\xrightarrow{}$ \cfbox{blue}{motion} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{motion sensor} $\xrightarrow{\text{motion}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}} &   2  & 1         \\ \hline
% 6   & \dashedbox{\framebox[1.1\width]{water sensor} $\xrightarrow{\text{wet}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}} $\xrightarrow{}$ \cfbox{blue}{illuminance} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{illum sensor} $\xrightarrow{\text{illum}>\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{curtain.close()}}$ \framebox[1.1\width]{curtain}} &   2  & 1         \\ \hline
% 7   & \dashedbox{\framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}<\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{heater}} $\xrightarrow{}$ \cfbox{blue}{smoke} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{smoke detector} $\xrightarrow{\text{detected}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}}$\xrightarrow{}$ \cfbox{blue}{illuminance}$\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{illum sensor} $\xrightarrow{\text{illum}>\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{curtain.close()}}$\framebox[1.1\width]{curtain}} &   3  & 2         \\ \hline
% \end{tabular}
% \caption{Chain of multiple events via hidden channels}
% \end{table*}


%-------following is the code for the second table--------
\begin{table*}[t]
\centering
\begin{tabular}[c]{|M{0.4cm}|M{16cm}|}
\hline
\textbf{No.} & \textbf{Event chain}  \\ \hline
1   
& \dashedbox{\framebox[1.1\width]{time}$\xrightarrow{}$\framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{toaster}} $\xrightarrow{}$ \textcolor{orange}{\framebox[1.1\width]{\textbf{smoke}}} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{smoke detector} $\xrightarrow{\text{detected}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{alarm.siren()}}$ \framebox[1.1\width]{alarm}} 
\\ \cline{2-2}
& $\circled{\small 1}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{smoke}}}
\xrightarrow{}\circled{\small 2}\xrightarrow{}\circled{\small 3}$ 
\\ \hline
2   
& \dashedbox{\framebox[1.1\width]{time}$\xrightarrow{}$\framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{heater}} $\xrightarrow{}$ \textcolor{orange}{\framebox[1.1\width]{\textbf{temperature}}} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}>\text{thresh}}$ \framebox[1.1\width]{hub} $\xrightarrow{\text{window.open()}}$ \framebox[1.1\width]{window}} 
\\ \cline{2-2}
& $\circled{\small 4}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{temperature}}}
\xrightarrow{}\circled{\small 5}\xrightarrow{}\circled{\small 6}$ 
\\ \hline
3   
& \dashedbox{\framebox[1.1\width]{presence sensor}$\xrightarrow{\text{not present}}$ \framebox[1.1\width]{hub}} $\xrightarrow{}$ \textcolor{orange}{\framebox[1.1\width]{\textbf{location mode}}} $\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{hub} $\xrightarrow{\text{switch.off()}}$ \framebox[1.1\width]{light}} 
\\ \cline{2-2}
& $\circled{\small 7}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{location mode}}}
\xrightarrow{}\circled{\small 8}$ 
\\ \hline
4   
& \dashedbox{\framebox[1.1\width]{humidity sensor} $\xrightarrow{\text{humidity}<\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{humidifier}} $\xrightarrow{}$ \textcolor{orange}{\framebox[1.1\width]{\textbf{humidity}}}
$\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{water sensor} $\xrightarrow{\text{wet}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}} 
\\ \cline{2-2}
& $\circled{\small 9}\xrightarrow{}\circled{\scriptsize 10}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{humidity}}}
\xrightarrow{}\circled{\scriptsize 11}\xrightarrow{}\circled{\scriptsize 12}$ 
\\ \hline
5   
& \dashedbox{\framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}<\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{fan}} $\xrightarrow{}$ 
\textcolor{orange}{\framebox[1.1\width]{\textbf{motion}}}
$\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{motion sensor} $\xrightarrow{\text{motion}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}} 
\\ \cline{2-2}
& $\circled{\small 5}\xrightarrow{}\circled{\scriptsize 13}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{motion}}}
\xrightarrow{}\circled{\scriptsize 14}\xrightarrow{}\circled{\scriptsize 12}$ 
\\ \hline
6   
& \dashedbox{\framebox[1.1\width]{water sensor} $\xrightarrow{\text{wet}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}} $\xrightarrow{}$ \textcolor{orange}{\framebox[1.1\width]{\textbf{illuminance}}}
$\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{illum sensor} $\xrightarrow{\text{illum}>\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{curtain.close()}}$ \framebox[1.1\width]{curtain}} 
\\ \cline{2-2}
& $\circled{\scriptsize 11}\xrightarrow{}\circled{\scriptsize 12}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{illuminance}}}
\xrightarrow{}\circled{\scriptsize 15}\xrightarrow{}\circled{\scriptsize 16}$ 
\\ \hline
7   
& \dashedbox{\framebox[1.1\width]{temp sensor} $\xrightarrow{\text{temp}<\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{heater}} $\xrightarrow{}$ 
\textcolor{orange}{\framebox[1.1\width]{\textbf{smoke}}}
$\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{smoke detector} $\xrightarrow{\text{detected}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{switch.on()}}$ \framebox[1.1\width]{light}}$\xrightarrow{}$ 
\textcolor{orange}{\framebox[1.1\width]{\textbf{illuminance}}}
$\xrightarrow{}$ \dashedbox{\framebox[1.1\width]{illum sensor} $\xrightarrow{\text{illum}>\text{thresh}}$ \framebox[1.1\width]{hub}$\xrightarrow{\text{curtain.close()}}$\framebox[1.1\width]{curtain}} 
\\ \cline{2-2}
& $\circled{\small 5}\xrightarrow{}\circled{\small 4}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{smoke}}}
\xrightarrow{}\circled{\small 2}\xrightarrow{}\circled{\scriptsize 12}\xrightarrow{}
\textcolor{orange}{\framebox[1.1\width]{\textbf{illuminance}}}
\xrightarrow{}\circled{\scriptsize 15}\xrightarrow{}\circled{\scriptsize 16}$ 
\\ \hline
\end{tabular}
\caption{Chain of multiple events via hidden channels}
\end{table*}
